Uplift Regression: The R Package tools4uplift

Uplift modeling aims at predicting the causal effect of an action such as a medical treatment or a marketing campaign on a particular individual, by taking into consideration the response to a treatment. The treatment group contains individuals who are subject to an action; a control group serves for comparison. Uplift modeling is used to order the individuals with respect to the value of a causal effect, e.g., positive, neutral, or negative. Though there are some computational methods available for uplift modeling, most of them exclude statistical regression models. The R Package tools4uplift intends to fill this gap. This package comprises tools for: i) quantization, ii) visualization, iii) feature selection, iv) parameter estimation and v) model validation.

==> old/Rdiag.tex <==


\begin{comment}
\begin{figure}%[H]
    \centering
    \begin{tikzpicture}[->,>=stealth',auto,node distance=1.5cm, scale=0.8, every node/.style={scale=0.8}]
    % Create an entity with ID node1, label "Fancy Node 1".
    % Default for children (ie. attributes) is to be a tree "growing up"
    % and having a distance of 3cm.
    %
    % 2 of these attributes do so, the 3rd's positioning is overridden.
    \node[entity] (QiniTable) {\code{QiniTable}}
        [grow=up,sibling distance=3cm]
        child[grow=left,level distance=3cm] {node[attribute] (QiniArea) {\code{QiniArea}}}
        child {node[attribute] (QiniBarPlot) {\code{QiniBarPlot}}}
        child[grow=right,level distance=3cm] {node[attribute] (QiniCurve) {\code{QiniCurve}}};
    %
    \node[entity] (DualUplift) [below = of QiniCurve] {\code{DualUplift}}
        [grow=down,sibling distance=3.5cm]
        child {node[attribute] (DualPredict) {\code{DualPredict}}};
    %    
    \node[entity] (InterUplift) [above left = of QiniBarPlot] {\code{InterUplift}}
        [grow=up,sibling distance=3.5cm]
        child {node[attribute] (InterPredict) {\code{InterPredict}}};
    %
    \node[relationship] (glmnet)  [above right  = of InterPredict] {\code{glmnet}}
        [grow=up,sibling distance=3.5cm]
        child {node[attribute] (LassoPath) {\code{LassoPath}}};
        
    \node[attribute] (BestFeatures) [above  = of LassoPath] {\code{BestFeatures}};
    % Draw an edge between two attributes
    \path (LassoPath) edge (BestFeatures);
     %    
    \node[relationship] (dplyr) [right = of glmnet] {\code{dplyr}}
        [grow=up,sibling distance=3.5cm]
        child {node[attribute] (SplitUplift) {\code{SplitUplift}}};
    % Draw an edge between two attributes
    % It is possible to use \draw as well
    \draw [->,black] (SplitUplift) to [out=90,in=0] (BestFeatures.east);
    \draw [->,black] (InterPredict.west) to [out=150,in=150] (BestFeatures);
    \draw [->,black] (QiniCurve.east) to [out=0,in=0] (DualPredict);
    \draw [->,black] (QiniCurve.east) to [out=0,in=0] (InterPredict);
    \draw [->,black] (QiniArea.west) to [out=180,in=180] (InterPredict);
    \draw [->,black] (QiniArea.west) to [out=180,in=180] (DualPredict);
    
    %    
    \node[entity] (BinUplift) [right = of SplitUplift] {\code{BinUplift}};
    \node[attribute] (BinUpliftEnhanced) [below = of BinUplift] {\code{BinUpliftEnhanced}};
    \draw [->,black] (BinUplift.west) to [out=180,in=180] (BinUpliftEnhanced);
    \node[entity] (SquareUplift) [below = of BinUpliftEnhanced] {\code{SquareUplift}};
    
    \end{tikzpicture}
    \caption{Diagram of function dependencies. Ellipses denote functions developed in the \pkg{tools4uplift} that are dependent on other functions. $A \longrightarrow B$ means that $B$ depends on $A$. Rectangles denote independent functions and diamonds denote pre-existing \proglang{R} libraries.}
    \label{fig:Rdiagram}
\end{figure}
\end{comment}

==> old/computation_old.tex <==
%In order to analyze our algorithms in terms of runtime, two simple experiments were performed. The experiments were run on a desktop PC with Intel Core i7-7700 CPU @ 3.60GHz with 16 GB of RAM and Windows 10 operating system. For the univariate quantization algorithm of Section~\ref{sec:manipulation}, Figure~\ref{fig:runtimebinning} shows the system runtime as a function of the number of split points to test at each node. For the bivariate quantization algorithm, the system runtime as a function of the number of rectangles is shown in Figure~\ref{fig:runtimesquares}. In both cases, we see that the algorithms are computationally efficient.

\begin{comment}
\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
            width=0.95\textwidth,
            height=0.5\textwidth,
            xtick={10,50,100,200,500,1000},
            ytick={0.00,0.25,0.50,0.75,1.00,1.25},
            xlabel={Number of splits (\code{n.split})},
            ylabel={\code{Sys.time} (in seconds)},
            legend style={at={(0.5,1)},
                anchor=north,legend columns=-1},
        ]
        %For n = 100
        \addplot table {
                        10 0.0411
                        50 0.0642
                        100 0.1073
                        200 0.2286
                        500 0.5475
                        1000 0.9466
                        };
        %For n = 200
        \addplot table {
                        10 0.0341
                        50 0.0832
                        100 0.0732
                        200 0.1735
                        500 0.3379
                        1000 0.9696
                        };
        %For n = 500
        \addplot[mark=+, dashed] 
                table {
                        10 0.0511
                        50 0.1023
                        100 0.1324
                        200 0.3820
                        500 0.6036
                        1000 1.0266
                        };
        %For n = 1000
        \addplot table {
                        10 0.0471
                        50 0.0892
                        100 0.1744
                        200 0.3471
                        500 0.7401
                        1000 1.2835
                        };
        \legend{$n=100$, $n=200$, $n=500$, $n=1000$}
    \end{axis}
    \end{tikzpicture}
    \caption{Runtimes (in seconds) of Algorithm~1 of the \code{BinUplift()} function (see Section \ref{sec:manipulation}) for univariate quantization of a continuous variable, as a function of the number of splits to test at each node of the decision tree. The different colored curves represent different sample sizes.}
    \label{fig:runtimebinning}
\end{figure}

\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
            width=0.95\textwidth,
            height=0.5\textwidth,
            xtick={4,16,25,100,225,625},
            ytick={0,0.1},
            xlabel={Number of squares (\code{n.split} $\times$ \code{n.split})},
            ylabel={\code{Sys.time} (in seconds)},
            legend style={at={(0.5,1)},
                anchor=north,legend columns=-1},
        ]
        %For n = 100
        \addplot table {
                        4 0.0342
                        16 0.0311
                        25 0.0291
                        100 0.0391
                        225 0.0511
                        %625 0.1003
                        };
        %For n = 200
        \addplot table {
                        4 0.0311
                        16 0.0381
                        25 0.0421
                        100 0.0401
                        225 0.0531
                        %625 0.1163
                        };
        %For n = 500
        \addplot[mark=+, dashed] 
                table {
                        4 0.0311
                        16 0.0311
                        25 0.0401
                        100 0.0461
                        225 0.0993
                        %625 0.1143
                        };
        
        %For n = 1000
        \addplot table {
                        4 0.0341
                        16 0.0311
                        25 0.0381
                        100 0.0561
                        225 0.0672
                        %625 0.1203
                        };
       
        \legend{$n=100$, $n=200$, $n=500$, $n=1000$}
    \end{axis}
    \end{tikzpicture}
    \caption{Runtimes (in seconds) of Algorithm~2 of the \code{SquareUplift()} function (see Section \ref{sec:manipulation}) for bivariate quantization of two continuous variables, as a function of the number of rectangles to use in order to estimate the uplift. The different colored curves represent different sample sizes. The maximum observed runtime in our experiment was $0.0993$ seconds.}
    \label{fig:runtimesquares}
\end{figure}
\end{comment}
